Closing the Gap: A User Study on the Real-world Usefulness of AI-powered Vulnerability Detection & Repair in the IDE

This paper presents the first empirical study of a vulnerability detection and fix tool with professional software developers on real projects that they own. We implemented DeepVulGuard, an IDE-integrated tool based on state-of-the-art detection and fix models, and show that it has promising performance on benchmarks of historic vulnerability data. DeepVulGuard scans code for vulnerabilities (including identifying the vulnerability type and vulnerable region of code), suggests fixes, provides natural-language explanations for alerts and fixes, leveraging chat interfaces. We recruited 17 professional software developers at Microsoft, observed their usage of the tool on their code, and conducted interviews to assess the tool's usefulness, speed, trust, relevance, and workflow integration. We also gathered detailed qualitative feedback on users' perceptions and their desired features. Study participants scanned a total of 24 projects, 6.9k files, and over 1.7 million lines of source code, and generated 170 alerts and 50 fix suggestions. We find that although state-of-the-art AI-powered detection and fix tools show promise, they are not yet practical for real-world use due to a high rate of false positives and non-applicable fixes. User feedback reveals several actionable pain points, ranging from incomplete context to lack of customization for the user's codebase. Additionally, we explore how AI features, including confidence scores, explanations, and chat interaction, can apply to vulnerability detection and fixing. Based on these insights, we offer practical recommendations for evaluating and deploying AI detection and fix models. Our code and data are available at https://doi.org/10.6084/m9.figshare.26367139.

==> background.tex <==
\section{Background}

\subsection{Transformer vulnerability detection models}

\ben{Transformer model architecture}

\ben{Pretraining}

\ben{Finetuning, classifier layer (generalize to $d+k$ logits)}

\subsection{IDE static analysis}

\ben{Copilot chat}

\ben{VSCode, extensions}

\ben{Findings from prior studies on static analysis}

==> old-lessons-learned.tex <==
\new{\takeaway{Current AI vulnerability detection and fix tools are not yet satisfactory, but developers remain eager to continue using them.}}
Our study shows that deep learning-based detection and fix tools hold promise.
% 
\tool{} and provided users with explanations and fix suggestions which they expressed were useful for understanding vulnerabilities and taking action to fix them.
By leveraging deep learning models to analyze code snippets, our tool could be set up quickly and run at a satisfactory speed for most users.

\ben{Bring back the suggestions about how to reduce FP.}
However, \tool{} has limitations that reduce its usefulness.
The main issue is an excessive number of false positives, which can arise from incorrectly recognizing vulnerable patterns or lacking context about a code snippet’s runtime environment or calling context.
While we explored a basic LLM-based filtering approach, improvements could be made by incorporating contextual information or providing examples of common false positives.
Additionally, our tool often could not suggest effective security fixes, which are complex and require a high degree of correctness. Chat interaction seems to be a promising method for iteratively producing applicable fixes.

% \wei{providing a takeaway message:
% Is it useful? yes/no: no
% accuracy? improve the model, 70\%
% tool features? improve the tool
% \\
% features x y z in \tool{} are useful
% \\
% features a b c would be useful but are not yet implemented
% }

% {\bf discussions}
% \ben{Discuss our findings. Below is a living outline of initial thoughts from our interviews so far.}

\smallheader{Recommendations for deploying AI models} \wei{We need to clean up this part to remove "obvious conclusions"}
Our findings suggest that combining models is a practical approach to addressing user requirements, as demonstrated by our novel LLM filtering technique.
Providing explanations and suggested fixes can be helpful, but it must be both concise and actionable.
We believe that ensuring that fixes are directly applicable without requiring syntax corrections would significantly improve their utility.
% \ben{Users have a high bar for applying security-related fix suggestions. Many proper security fixes are complex or require changing multiple sections of code.}
% \ben{P12 interestingly remarked that, since they triggered a scan on a directory, they expected the model to use the context of the entire directory.}
Additionally, model-generated localizations may not always align with user intentions and should be post-processed to better meet user needs.
Finally, users expressed a desire to configure the tool, including the ability to adjust detection sensitivity and ruleset, and customize the fix, e.g. whether they see placeholder fixes.

\smallheader{Recommendations for presenting model outputs}
Based on our findings, we recommend several key considerations for presenting model outputs in vulnerability detection tools. First, incorrect or partially correct results can still be valuable by prompting users to consider important issues or providing a starting point for remediation. \wei{do we mentioned this point before anywhere?}
Second, the user interface plays a crucial role, often as significant as the accuracy of the results.
\new{Some participants who found the tool potentially useful rated it poorly, citing workflow disruptions due to the need for manually-triggered scans or overly verbose vulnerability alerts.
% This indicates that an intuitive interface is essential for adoption.
}
Third, brevity is important; users preferred concise summaries over lengthy explanations, with options for extended text when they wanted to investigate further.
Lastly, participants frequently misinterpreted confidence scores as severity scores, using them to prioritize alerts. We need to introduce additional metrics, such as bug severity based on vulnerability type and location, to rank the issues accurately. %highlighting the need for clear communication of the meaning of reported metrics.
% \ben{Incorrect results can be useful, for example, if they make the user think about an important issue or provide the start to remediation.}
% \ben{User interface of a tool matters nearly as much as the correctness of the results. Even some participants who thought the tool would be useful rated it low for workflow and stated that they wouldn't use it for that reason.}
% \ben{Brevity is important. Users often could not/did not want to absorb a large amount of text, and often pointed out that they wish that the tool's messages could be rephrased to offer a summary and extended text for further reading.}
% \ben{Participants sometimes interpreted the confidence 
% score as a severity score. They most often used the score to prioritize the alerts.}

\smallheader{Recommendations for model evaluations}
For model evaluations, it is crucial to align evaluation settings with real deployment scenarios to get a desired false positive and false negative balance.

% 0.5\% false positive rate is the threshold recommended by the state of the art PrimeVul evaluation method
\new{\citet{primevul} introduced the Vulnerability Detection Score (VD-S), and utilized a threshold of 0.5\% false positive rate (FPR). Although this metric is promising,} our results suggest that developers will tolerate a higher FPR and may lose trust in the tool if too few alerts are surfaced. This suggests the need to adopt a more realistic threshold for evaluation metrics.

%\wei{Who said we need 0.5\% While PrimeVul's vulnerability detection score (VDS)~\cite{primevul} is a promising metric, the tolerance level of 0.5\% false positives appears too stringent for our security application based on our data.}
% 
%Although false positives were a significant issue for our tool's effectiveness, several participants were willing to tolerate some false positives in exchange for valid results, with 

For example, one participant stated, \quot{Like any of these kind of static analysis tools, there can be plenty of false positives, but every now and then there'll be a nugget of gold I'm looking at.}
Reporting too few false negatives for new or untested code that users expect to be insecure can undermine trust in the tool. As noted by one participant, \quot{You maybe set the bar a little bit too high... if you have more issues I will have more confidence because, if you tell me that 20 or 30 files in [a simple, untested application] don't have an issue at all, I don't have confidence in this result.}
%Based on these findings, aligning model evaluations with user requirements will allow effective model development and ensure real quality improvements in tool usage.
% \ben{Evaluation settings should be close to the deployment scenario}
% \ben{PrimeVul's vulnerability detection score (VDS) is a good idea, but they set tolerance to 0.5\%, which seems too low for our security application based on our data; although false positives were a blocker for our tool's usefulness, several participants stated that they were found would accept a number of false positives as long as they got some valid results -- \quot{Like any of these kind of static analysis tools, there can be plenty of false positives, but every now and then there'll be a nugget of gold I'm looking at}.
% Reporting too few false negatives for code the user doesn't expect to be secure can also degrade trust in the tool, as stated: \quot{You maybe set the bar a little bit too high... if you have more issues I will have more confidence because, if you tell me that 20 or 30 files in [a simple, untested application] don't have an issue at all, I don't have confidence in this result.}}

\ben{Mention about the commonality of wrong approach motivating better evaluations for fixes}

\smallheader{Recommendations for further research}
As the first of its kind, our user study revealed several promising areas for further investigation.
% \ben{Background scan}
First, users wanted the tool to automatically scan code as they edited, rather than requiring manual triggers. \new{Future research should explore the tool's effectiveness while scanning incomplete code,
% \wei{the tool's integration with IDE to schedule automatic scanning},
the impact of automatic scanning on runtime speed, and optimal timing for scanning code and presenting alerts.}
% \ben{The role of explanations and chatbots}
Second, while we briefly touched on explanation and chat capabilities, future research can examine how different explanations affect developers' understanding security vulnerabilities and how chat interaction can address limitations in the current fix model for complex, multi-site fixes.
% \ben{Configuring the models}
Lastly, we did not explore the effects of tool configuration and alert suppression, but users indicated that these settings could enhance the tool's long-term utility. 
The VS code plugin we developed enables easy collection of tool usage and feedback data as developers continue to use it during organic development. Such longitudinal studies on tool usage patterns and configurations would provide valuable insights for improving adoption and effectiveness.
% These provide valuable and concrete directions for future research.

==> old-model-architecture.tex <==

We implemented our detection model (which we call \toolDetect{}) by fine-tuning CodeBERT~\cite{codebert}, following the procedure and using the dataset introduced in \citet{edittime}. We chose this model because it is suited to Edit-Time vulnerability detection, localization, and bug-type prediction, while other state-of-the-art models we considered~\cite{linevul,deepdfa} are trained on and primarily intended for complete code snippets without the ability to both localize lines and predict a specific bug type.
We fine-tuned \toolDetect{} for \textit{multi-task prediction}. For each given code snippet, it predicts: (1) whether the snippet contains a vulnerability, (2) whether any specific tokens in the snippet contain a vulnerability, and (3) the type of the vulnerability.
\Cref{fig:models-overview} shows an overview of our detection model approach. We replaced the final classifier layer (normally performing binary classification) with a layer of size ($d + k$), where $d$ is the number of tokens in the context window (512 for CodeBERT) and $k$ is the number of bug types in our training dataset (27 in our case), followed by a softmax layer. During training, we labeled the tokens (\ben{where did we get the ground-truth for labeling the tokens?}) with 1 when the code contained a vulnerability related to that token and 0 otherwise, did likewise for the bug types, and trained the model to jointly predict these $512 + 27 = 539$ classes for each example.
To train the model, we used a dataset collected using the same methodology as \citet{edittime}, consisting of vulnerable code snippets in public
GitHub repositories detected by CodeQL.

% \begin{table}[h]
%     \centering
%     \caption{Statistics of our training dataset. \ben{Move to appendix.}}
%     \begin{tabular}{lrrr}
%     \toprule
%         Language & \# CWEs & \# Vulnerable & \# Non-Vulnerable \\
%     \midrule
%         C/C++ & XX & XX & XX \\
%         C\# & XX & XX & XX \\
%         Go & XX & XX & XX \\
%         Java & XX & XX & XX \\
%         JavaScript/TypeScript & XX & XX & XX \\
%         Python & XX & XX & XX \\
%         Ruby & XX & XX & XX \\
%     \bottomrule
%     \end{tabular}
%     \label{fig:dataset-statistics}
% \end{table}

% \Cref{fig:dataset-statistics} shows the statistics of our training dataset.
We trained \toolDetect{} on a dataset containing XXX code snippets in seven languages (C/C++, C\#, Go, Java, JavaScript/TypeScript, Python, and Ruby), including bug types corresponding to 27 CodeQL rules marked as impactful in the CWE database~\cite{cwe-database}, including Path Injection, SQL injection, Cross-Site Scripting (XSS), URL Redirection, Hard-coded Credentials, and Plain-Text Logging of Sensitive Data.
% \ben{TODO: Describe the dataset collection or say we re-used the dataset from the prior paper.}
We found that this multi-task fine-tuning was effective for providing localization and bug type classification, allowing the model to attain XXX loss and XXX validation accuracy during training.

\ben{Summarize and move to appendix.}
\wei{{\bf GPT filtering}}
During our experiments, we found that \toolDetect{} tended to make several cases of spurious predictions on certain bugs such as hard-coded credentials, plain-text logging of sensitive data, and SQL injection. These represent cases where correct detection requires nuanced decisions about the involved code and identifier names and may benefit from the emergent capabilities and greater capacity of large language models (LLMs) which might not be available for small language models (SLMs) similar to the scale of CodeBERT.
We also found that LLMs predicted more conservatively than fine-tuned SLMs, resulting in higher precision but lower recall \ben{Needs experimental support}.
% , often generating responses along the lines of ``As a large language model, I do not have enough information...''
However, many capable LLMs contain billions of parameters~\cite{scaling-laws} (compared to 125 million for our fine-tuned CodeBERT model~\cite{codebert}) and the closed-source weights cannot be optimized for production, which introduces latency which is unacceptable for scanning large corpora of source code; scalability was identified as a pain point for static analysis tools \cite{johnson_whydont_2013,christakis_whatdeveloperswantandneed_2016} \ben{TODO: check citation}.
To leverage the complementary benefits of both approaches, we used \toolDetect{} to detect potential vulnerabilities, then used an LLM to filter all vulnerable predictions.
We found that the LLM filter improved the precision by up to 20\% (see \Cref{sec:benchmarking}).

\begin{figure}[htbp]
    \centering
    \caption{The prompt used by \toolFix{}.}
\begin{minted}
[
framesep=2mm,
baselinestretch=1.2,
bgcolor=LightGray,
fontsize=\footnotesize,
breaklines
]
{python}
'''
A static analyzer has identified a {rule_id} security vulnerability in the {language} method below:

```
{method}
```

The SARIF result message is as follows: {message}

{description}

Write a fixed version of the method above and wrap it in triple backticks, then explain why your version addresses the problem.
'''
\end{minted}
    \label{fig:fix-prompt}
\end{figure}

We implemented our fix model (\toolFix{}) using GPT-4~\cite{gpt4} with specialized prompts shown in \Cref{fig:fix-prompt}. We chose this model because of its demonstrated high performance for generating bug-fixes and natural-language explanations, and the flexibility and generalization of LLM prompting approaches compared to fine-tuning \ben{Any citation available?}.
We prompted the model with instructions and the context surrounding the vulnerability alert; if the alert appears inside a function, we provide the entire function, and if it appears in a class or file, we provide the entire file.
\ben{Any prior approaches we can cite?}
\ben{Any postprocessing to insert the fix?}
\wei{We need to cut down this section}


==> open-questions.tex <==
\ben{Open questions, consider adding:}

\ben{Hypothesis: Participants were much more likely to judge the tool to be useful when they got a few true positives.}
\ben{What bug types performed best/worst?}
\ben{How did the model perform on different languages, such as C\# vs. TS?}

\ben{Hypothesis: Users who use chat tools are more likely to pay attention to explanations and chat.}

